The evolutionary roads leading to low effective spins, high black hole masses, and O1/O2 rates of LIGO/Virgo binary black holes

All ten LIGO/Virgo binary black hole (BH-BH) coalescences reported from the O1/O2 runs have near zero effective spins. There are only three potential explanations of this fact. If the BH spin magnitudes are large then (i) either both BH spin vectors must be nearly in the orbital plane or (ii) the spin angular momenta of the BHs must be oppositely directed and similar in magnitude. Or, (iii) the BH spin magnitudes are small. We test the third hypothesis within the framework of the classical isolated binary evolution scenario of the BH-BH merger formation. We test three models of angular momentum transport in massive stars: a mildly efficient transport by meridional currents (as employed in the Geneva code), an efficient transport by the Tayler-Spruit magnetic dynamo (as implemented in the MESA code), and a very-efficient transport (as proposed by Fuller et al.) to calculate natal BH spins. We allow for binary evolution to increase the BH spins through accretion and account for the potential spin-up of stars through tidal interactions. Additionally, we update the calculations of the stellar-origin BH masses, include revisions to the history of star formation and to the chemical evolution across cosmic time. We find that we can match simultaneously the observed BH-BH merger rate density, BH masses, and effective spins. Models with efficient angular momentum transport are favored. The updated stellar-mass weighted gas-phase metallicity evolution now used in our models appears to be a key in better reproducing the LIGO/Virgo merger rate estimate. Mass losses during the pair-instability pulsation supernova phase are likely overestimated if the merger GW170729 hosts a BH more massive than 50 Msun. We also estimate rate of BH-NS mergers from recent LIGO/Virgo observations. Our updated models of BH-BH, BH-NS and NS-NS mergers are now publicly available at www.syntheticuniverse.org.

==> aa.tex <==

The origin of low effective spins in LIGO/Virgo binary black hole mergers


      Krzysztof Belczynski


All of the ten LIGO/Virgo binary black hole (BH-BH) merger detections to date 
have low values for their effective spins. There are only three potential
explanations of this fact. If  BH spin magnitudes are large then (i) both BH 
spin vectors must lie in/near orbital plane or (ii) they must be pointing in 
opposite directions. Or (iii) BH spin magnitudes are small.  
%
We test the third hypothesis within the framework of the classical binary evolution 
scenario of the formation of BH-BH mergers. We test three models of angular 
momentum transport in massive stars: the Geneva model (mildly efficient transport), 
the MESA model (efficient transport), and the Fuller model (super-efficient transport) 
to calculate natal BH spins. We allow for binary evolution to increase the BH spins 
through accretion and account for the potential spin-up of stars through tidal 
interactions. Additionally, we update calculations of stellar-origin BH masses, 
include revisions to the cosmic history of  star formation at high redshifts, and model 
the evolution of the mean  metallicity of star-forming gas across cosmic time. 
%
We find that we can match simultaneously the observed BH-BH merger rate density,
BH masses, and effective spins. Models with efficient angular momentum transport 
are favored. The new stellar-mass weighted gas-phase metallicity used in our model appears 
to be key in better reproducing the LIGO/Virgo merger rate estimates.
Mass losses during the pair-instabilty pulsation supernova phase are likely
overestimated if the merger GW170729 hosts a BH more massive than 50 Msun.
%
If in fact angular momentum transport in massive stars is efficient, then any 
observation of a highly spinning BH would indicate either a very effective tidal
spin up of the progenitor star (e.g., homogeneous evolution, high-mass X-ray 
binary formation through case A mass transfer), or significant  gas accretion 
by the hole  (e.g., a low/intermediate-mass X-ray binary phase), or  BH formation 
thorugh the merger of two BHs (e.g, in a dense stellar cluster). 

